Parallel Derandomization for Coloring

Graph coloring problems are among the most fundamental problems in parallel and distributed computing, and have been studied extensively in both settings. In this context, designing efficient deterministic algorithms for these problems has been found particularly challenging. In this work we consider this challenge, and design a novel framework for derandomizing algorithms for coloring-type problems in the Massively Parallel Computation (MPC) model with sublinear space. We give an application of this framework by showing that a recent $(degree+1)$-list coloring algorithm by Halldorsson et al. (STOC'22) in the LOCAL model of distributed computation can be translated to the MPC model and efficiently derandomized. Our algorithm runs in $O(\log \log \log n)$ rounds, which matches the complexity of the state of the art algorithm for the $(\Delta + 1)$-coloring problem.

==> parts/d1lc_deterministic.tex <==
%\section{Derandomization of Algorithm for Low-Degree Instances}
\section{Derandomization for Low-Degree}
\label{sec:deterministic_d1lc}

In this section, we give a deterministic \MPC algorithm, for \DILC for a graph $G$ with maximum degree at most $n^{7\delta}$, that takes $O(\log \log \log n)$ rounds on an \MPC with $\lspace=O(n^\phi)$ and $O(n^{1+\phi})$ global space~\footnote{The number of edges is always at most $O(n^{1+\phi})$.}. This is possible due to the simulation of  deterministic steps in \cite{hknt_local_d1lc} when the maximum degree is at most $\sqrt{\lspace}$ as discussed in \Cref{sec:randomized-d1lc} and the fact that the randomized steps in \cite{hknt_local_d1lc} can be efficiently derandomized. In particular, we will discuss the derandomization of \textsc{TryRandomColor}(\Cref{alg:try_random_color}), \textsc{SlackColor} (\Cref{alg:slack_color}), {\sc GenerateSlack} (\Cref{alg:generate_slack}), \textsc{PutAside} (\Cref{alg:put-aside}) and \textsc{SyncColorTrial} (\Cref{alg:synch}) by proving that all of them are $(O(\log ^*n),\Delta)$-round  distributed procedures and arguing that such procedures can be efficiently derandomized by using pseudorandom generators.  We can show that, in one iteration with $O(\log^* n)$ rounds, the number of uncolored nodes will be reduced by a factor of $n^{\Omega(1)}$ (that are deferred to be colored in the later iterations). So, by repeating the process for $O(1)$ iterations, we have $O(\log n)$ nodes left to be colored. Another thing to note that, we are considering the algorithm of \Cref{sec:overview_of_hknt} here when the degree of the nodes is at least $\log ^7 n$. So, we always defer the coloring of the nodes whose degree is at most $\log ^7 n$. So, at the end we have a graph (of at most $n$ nodes) having maximum degree $\log ^7 n$. Note that this can be colored in $O(\log \log \log n)$ rounds due to a result of \cite{CDP21}.

 In this section, graph $G$ is often is not clear from the context. So, we use $n_G$ to denote the number of nodes in $G$. For a node $v$, $N_G(v)$ denote the set of neighbors of $v$ in $G$ and $d_G(v)$ denotes the degree of $v$ in $G$. We denote the maximum degree of any node in $G$ by $\Delta_G$. For a node $v$ and $c \in \mathbb{N}$, $N^c_G(v)$ denotes the nodes in the $c$-hop neighborhood of $v$.

\subsection{Normal distributed procedures}

First, we define the notion of $(c,\Delta_G)$-round randomized distributed procedure.

\begin{definition}\label{prng-derandomizable}
A \emph{normal $(c,\Delta_G)$-round distributed procedure} running on a graph $G$, of maximum degree \emph{at most} $\Delta_G$, is a procedure in the randomized \LOCAL model satisfying the following criteria:

\begin{itemize}
\item The procedure takes $c$ rounds of \LOCAL.
\item At the beginning of the procedure, nodes $v$ have $O(\Delta_G^c)$-word sets of input information $\textsc{In}_v$ associated with them.
\item During the procedure, nodes only use information from their $c$-hop neighborhood (i.e. from $\textsc{In}_v \cup \bigcup_{u\in N^c_G(v)} \textsc{In}_u\}$ and $O(\Delta_G^{2c})$ random bits, and perform $O(\Delta_G^{8c})$ computation. %\gopi{$N^c_G(v)$ denotes the set of vertices that are with in $c$-hop neighborhood of $v$.}
\item The output of the procedure is a new $O(\Delta_G^c)$-word set of output information $\textsc{Out}_v$ for each node.
\item The procedure has a `success property' (computable with $O(\Delta_G^{8c})$ computation) that determines whether it has been successful for a particular node, based on the output information of that node and its $c$-hop neighborhood (formally, $\textsc{SP} : \textsc{Out}_v \cup \bigcup_{u\in N^c_G(v)} \textsc{Out}_u \rightarrow \{T,F\}$).
\item At the end of the procedure, then for any node $v$, $$\Prob{\textsc{SP}(\textsc{Out}_v \cup \bigcup_{u\in N^c_G(v)} \textsc{Out}_u ) = T} \ge 1-\frac{1}{2n_G}.$$
%\gopi{What does $n_G$ here? Is it the number of vertices in $G$? Should it be $n_G^{\Omega(1)}$?}
\item Each success property is such that `deferring' nodes to be dealt with later cannot cause the property to become unsatisfied. That is, if we denote by $\textsc{Defer}_w$ a special status indicating that $w$ is to be deferred (which is not to be conferred by the procedure itself), then adding $\textsc{Defer}_w$ to $w$'s output information should not cause any other nodes' success properties to become unsatisfied. Formally:

$$
 \textsc{SP}\left(\textsc{Out}_v \cup \bigcup_{u\in N^c_G(v)} \textsc{Out}_u \right) = T  
\Rightarrow \forall w\in N^c_G(v), \textsc{SP}\left(\textsc{Out}_v\cup \{\textsc{Defer}_w\} \cup \bigcup_{u\in N^c_G(v)} \textsc{Out}_u \right) = T\enspace.
$$

\end{itemize}
\end{definition}

%\gopi{Shall we add some sentences here?}
In the following lemma, we show that a number of randomized subroutines of \cite{hknt_local_d1lc} are in fact normal $(O(1), \Delta_G)$-round distributed procedures. Under these circumstances, we can use a pseudorandom generator, combined with the method of conditional expectations, to derandomize the algorithm. The details of PRG and the derandomization  will be discussed in \Cref{sec:derand}.
\begin{lemma}
\label{lem:derandomizable-subroutines}
The subroutines
{\sc TryRandomColor} (\Cref{alg:try_random_color}),
{\sc GenerateSlack} (\Cref{alg:generate_slack}),
{\sc PutAside} (\Cref{alg:put-aside}),
and {\sc SynchColorTrial} (\Cref{alg:synch})
are all normal $(O(1), \Delta_{G})$-round distributed procedures. The subroutine {\sc SlackColor} (\Cref{alg:slack_color}) consists of a sequence of $O(\log^* \Delta)$ normal $(O(1), \Delta_G)$-round distributed procedures.
\end{lemma}

\begin{proof}
First, we note that at the start of any algorithm, nodes may be assumed to have information about which sets they are members of ($V_{\text{sparse}}$, $V_{\text{uneven}}$, etc.), as by earlier simulation arguments ({see \Cref{obs:spse}}) this can be computed in $O(1)$ rounds in \LOCAL (and \MPC, for low enough degree). We may also assume that nodes have information about the value of any of the parameters in \Cref{def:parameters} for themselves and any of their neighbours ({see \Cref{lem:computing_parameters}}). Note that this is, in total, $O(\Delta_{G}^2)$ words of information for each node $v$: a constant number of words for each parameter, $O(\Delta_{G})$ words for set membership, multiplied by the number of neighbors of $v$, which is $O(\Delta_{G})$.

We look at each in turn:
\begin{itemize}
    \item \textbf{\sc TryRandomColor}: The procedure takes $O(1)$ rounds of \LOCAL. Nodes need no other words of input information. Nodes only use information from their neighbors, and each node uses $O(\log \Delta_{G})$ random bits to select a color from its palette. Note that the computation is $O(\Delta_{G})$. The output information is either a color with which $v$ has permanently colored itself, or {\sc Fail} if it does not color itself: this is clearly $O(\Delta_{G})$ words of information. The success property is that the slack of a node increases from $c \cdot d_{G}(v)$ for some constant $c$ to $2 \cdot d_{G}(v)$ \cite[Lemma~26]{hknt_local_d1lc}. This is computable in time linear in the degree of a node and based only on the output of the immediate neighbors of a node. The property succeeds for each node with probability $p=\exp(\Omega(s(v)))$, and by our precondition, $s(v)$ is at least polylogarithmic so this is with high probability. Nodes deferring does not affect the algorithm, since this creates at least as much as slack as it would if all nodes participated.

    \item \textbf{\sc GenerateSlack}: This takes $O(1)$ rounds of \LOCAL and nodes need no other information at the beginning of the procedure. During the procedure, nodes only use information from their neighbors and $\widetilde{O}(\Delta_{G})$ random bits (to determine whether the node is sampled and if so, what color is attempted). The output of the procedure is either the color with which $v$ permanently colored itself, or {\sc Fail}. The success of the procedure is quite complicated: depending on the type of node, a different guarantee on the eventual slack is required. We note, however, that these guarantees all succeed with high probability and are computable using only information in the immediate neighborhood of $v$ \cite[Lemmas~10, 11, 13, 15, 17, 18]{hknt_local_d1lc}. Deferring nodes creates temporary slack and so does not hurt the procedure.

    \item \textbf{\sc PutAside}: The algorithm consists of $1$ round of \LOCAL, and nodes need no additional information. During the procedure, nodes only use information from their neighbours, and use $O(\polylog(n)) \in O(\Delta_{G})$ (by construction) random bits to independently sample nodes into $S_C$. The output of the procedure is one word (whether $v \in P_C$). A node succeeds if the put-aside set of the almost-clique containing it (say $C$) satisfies $\size{P_C} = \Omega(\ell^2)$ for some polylogarithmic $\ell$ \cite[Lemma~5]{hknt_local_d1lc}. This can be checked using the $2$-hop neighborhood of $v$ because the diameter of $C$ is at most $2$. The property succeeds with high probability. If we defer nodes then this can hurt the size of the put-aside per se, however this is not an issue: the fact that we are deferring nodes creates the necessary slack that the put-aside set would be creating anyway. We have to be careful however, to color the deferred nodes \emph{after} the put-aside set, otherwise we lose the property that the put-aside sets in different almost-cliques are independent.

    \item \textbf{\sc SynchColorTrial}: This procedure takes $1$ round of \LOCAL. Nodes need no additional information about their neighborhood beforehand. Nodes only use information from their immediate neighbors during the procedure (since leader $x_C$ neighbors all nodes in the set of inliers $I_C$), and in the worst case (i.e.~if the node in question is $x_C$), nodes need $\widetilde{O}(\Delta_{G})$ random bits to permute their palette. The output of the procedure for a node $v \in I_C$ for some $C$ is either a color in $\Psi_v$ or {\sc Fail}. The success property for the procedure is that, for the almost-clique $C$ that $v$ is in, the number of nodes that return {\sc Fail} is bounded by $O(t)$, where $t$ is some polylogarithmic value \cite[Lemma~7]{hknt_local_d1lc}. This happens with high probability ($\exp(-t)$). Nodes dropping out can only help the algorithm, as they are not counted as nodes which fail to be colored. 
    
    \item \textbf{\sc SlackColor}:  There are three parts to the algorithm. First, {\sc TryRandomColor} is called in order to amplify the slack of each node (which is linear in the degree: a prerequisite of {\sc SlackColor}). Then two loops of {\sc MultiTrial} instances are run.\\
    The $O(1)$ calls to {\sc TryRandomColor} are normal $(O(1), \Delta_{G})$-distributed procedures by the item above.\\
    Each iteration of the first for-loop of executions of {\sc MultiTrial} takes $O(1)$ \LOCAL rounds. Nodes need no additional input information. During the execution of the loop, nodes only use information from their immediate neighbors, and only use $O(\Delta_{G})$ random bits to select a subset of their palette. The output of the procedure for $v$ is either a color in $\Psi_v$ or {\sc Fail}, which is one word. Nodes succeed (with high probability) if $d(v) \le \slack{v}/\min(2^{x_i},\rho^\kappa)$ \cite[Lemma~27]{hknt_local_d1lc}. This is, again, computable using only the output of the node and output information of the immediate neighborhood. Nodes deferring reduce the degree (temporarily), and so they cannot cause the property to be unsatisfied.\\
    The second for-loop of {\sc MultiTrial} instances are normal distributed procedures for the same reason: the success property is $d(v) \le \slack{v}/\min(\rho^{(i+1) \cdot \kappa},\rho)$, and also satisfies the requirements of \Cref{prng-derandomizable}. So, overall \textbf{\sc SlackColor} consists of a sequence of $O(\log^* \Delta)$ normal $(O(1), \Delta_G)$-round distributed procedures.\qedhere

\end{itemize}
\end{proof}


%\subsection{Pseudorandom generators and derandomization in sublinear \MPC}
\subsection{PRGs and derandomization}\label{sec:derand}

A \emph{Pseudorandom Generator (PRG)} is a function that takes a short \emph{random seed} and produces a longer string of \emph{pseudorandom} bits, which are computationally indistinguishable from truly random bits. We use the following definition from \cite{Vadhan12} for indistinguishability:%\Anote{This definition may look a bit cryptic; it's only for decision algorithm (for otherwise notion $T(X)=1$ wouldn't make much sense), etc. But maybe it's OK. Peter - I added defining the algorithm as a function to $\{0,1\}$; is that better?}

\begin{definition}%[Computational indistinguishability, Definition 7.1 in \cite{Vadhan12}]
[Definition 7.1 in \cite{Vadhan12}]
\label{def:computational-indistinguishability}
Random variables $X$ and $Y$ taking values in $\{0,1\}^m$ are $(t,\eps)$ \textbf{indistinguishable} if for every non-uniform algorithm $T:\{0,1\}^m\rightarrow \{0,1\}$ running in time at most $t$, we have $|\Pr[T(X)=1]-\Pr[T(Y)=1]| \le \eps$.
\end{definition}
%\gopi{Shall we define what is non-uniform algorithm?}\Artur{No}

Let $U_k$ denote a random variable generated uniformly at random from $\{0,1\}^k$. Then pseudorandom generators are defined as follows:

\begin{definition}[PRG, Definition 7.3 in \cite{Vadhan12}]
\label{def:PRG}
A deterministic function $\mathcal{G}:\{0,1\}^d \to \{0,1\}^m$ is an \textbf{$(t,\eps)$ pseudorandom generator (PRG)} if (1) $d < m$, and (2) $\mathcal{G}(U_d)$ and $U_m$ are $(t,\eps)$ indistinguishable.%\gopi{what does $U_k$ denote here?}
\end{definition}

A simple application of the probabilistic method can show the existence of PRGs with optimal parameters:

\begin{proposition}[Proposition 7.8 in \cite{Vadhan12}]
\label{prop:perfect-PRG}
For all $t \in \mathbb{N}$ and $\eps>0$, there exists a (non-explicit) $(t,\eps)$ pseudorandom generator $\mathcal{G}: \{0,1\}^d \to \{0,1\}^t$ with seed length $d = \Theta(\log t+\log(1/\eps))$.
\end{proposition}

As shown in \cite{CDPcompstab}, such a PRG can be computed using relatively low space (but exponential computation).

\begin{lemma}[Lemma 35 of \cite{CDPcompstab}, arXiv version]
\label{lem:prg-alg}
For all $t \in \mathbb{N}$ and $\eps>0$, there exists an algorithm for computing the $(t,\eps)$ PRG of \Cref{prop:perfect-PRG} in time $\exp(poly(t/\eps))$ and space $poly(t/\eps)$.
\end{lemma}

For any integer $k\in \mathbb{N}$, let $G^k$ be the $k$-power of $G$, that is, $G^k$ is the graph having the same node set as $G$ and any pair of nodes at a distance at most $k$ in $G$ form an edge in $G^k$.

\begin{lemma}\label{lem:phasederand}
There is a constant $C$ such that, given an $O(\Delta_G^{8c})$-coloring of $G^{4c}$, any normal $(c,\Delta_G)$-round distributed procedure on a graph $G$ can be derandomized in $O(c)$ rounds of \MPC, using $\lspace=O(\Delta_G^{cC})$ space per machine and global $O(n_G \Delta_G^{cC})$, with the following properties:

\begin{itemize}
\item At most $\frac 12+n_G \Delta_G^{-11c}$ nodes are deferred.
\item All non-deferred nodes $v$ satisfy the success property.
\end{itemize}
\end{lemma}

\begin{proof}
First, for each node $v$ we collect the input information of its $8c$-hop neighborhood ($\textsc{In}_v \cup \bigcup_{u\in N^c_G(v)} \textsc{In}_u$) to a dedicated machine. This takes $c$ rounds, and requires $O(\Delta_G^{8c} \cdot \Delta_G^c) = O(\Delta_G^{11c})$ space per machine and $O(n_G \Delta_G^{11c})$ global space. Our aim is then to simulate the procedure using randomness produced by the $(\Delta_G^{11c}, \Delta_G^{-11c})$ PRG implied by \Cref{prop:perfect-PRG}. This PRG has seed length $d = \Theta(\log \Delta_G)$ and requires $poly(\Delta_G^{11c})$ space to construct and store. We choose $C$ so that this $poly(\Delta_G^{11c})$ term is $O(\Delta_G^{cC})$.

The PRG, when evaluated on a seed, produces a string of $\Delta_G^{11c}$ pseudorandom bits. We use the provided $O(\Delta_G^{8c})$-coloring of $G^{4c}$ to split this string into the input randomness for each node. By definition of a normal $(c,\Delta_G)$-round distributed procedure, each node requires $O(\Delta_G^{2c})$ random bits, and we provide a node colored $i$ in the $O(\Delta_G^{8c})$-coloring with the $i^{th}$ chunk of $O(\Delta_G^{2c})$ bits from the PRG's output. This means that any pair of nodes within distance $4c$ receive disjoint chunks of pseudorandom bits.

The output of the PRG under a random seed is $(\Delta_G^{11c},\Delta_G^{-11c})$ indistinguishable from a uniform distribution. Consider the process of simulating the procedure for all nodes within distance $c$ of a node $v$, and then evaluating the success property $\textsc{SP}(\textsc{Out}_v \cup \bigcup_{u\in N^c_G(v)} \textsc{Out}_u ) $. By definition of a normal $(c,\Delta_G)$-round distrib\-ut\-ed procedure, this combined process requires $O(\Delta_G^{9c})$ computation, and depends on the input information and randomness of nodes up to distance $2c$ from $v$ (and note that all nodes within this radius receive different chunks of the PRG's output as their pseudorandom bits). This combined process can therefore be run on one \MPC machine. Furthermore, it can be considered a non-uniform algorithm using at most $\Delta_G^{9c}$ computation, and so is `fooled' by the PRG. This means that the output ($T$ or $F$, indicating whether the success property is satisfied) at $v$ differs with probability at most $\Delta_G^{-11c}$ from what it would be under full randomness. That is, the output will be $F$ with probability at most $\frac{1}{2n_G}+ \Delta_G^{-11c}$.

The expected number of nodes who do not satisfy the success property, when simulating the procedure using the PRG with a random seed, is therefore at most $\frac 12+n_G \Delta_G^{-11c}$. Since this value is an aggregate of functions computable by individual machines, using the method of conditional expectations (as implemented for low-space MPC in \cite{CDPsparse,CDP20}) we can deterministically select a seed for the PRG for which the number of nodes which do not satisfy the success property is at most its expectation (i.e. at most $\frac 12+n_G \Delta_G^{-11c}$), in $O(1)$ rounds.

Then, we simply mark the nodes which do not satisfy the success property as deferred. In doing so, we meet the conditions of the lemma.
\end{proof}

\begin{lemma}\label{lem:fullderand}
There is a constant $C$ such that, given an $O(\Delta_G^{8c})$-coloring of $G^{4c}$, any normal $(c,\Delta_G)$-round distributed procedure on a graph $G$ with $\Delta_G \le n^{7\delta}$ can be derandomized in $O(c)$ rounds of \MPC, using $\lspace=O( n^{7\delta cC})$ space per machine and global space $O(n_G \cdot n^{7\delta cC})$, with all nodes satisfying the success condition of the procedure.
\end{lemma}

\begin{proof}
We repeatedly apply \Cref{lem:phasederand} to the graph induced by the deferred nodes, in each case using $\Delta_G = n^{7\delta}$ as an upper bound on the maximum degree (even though the actual maximum degree may be significantly lower). After $r$ iterations of this, the number of remaining deferred nodes is at most $\frac 34 + n\cdot n^{-11cr\cdot7\delta}$. Taking $r=1/\delta$ (which is $O(1)$), we then have fewer than $1$ remaining deferred node, i.e.~all nodes satisfy the success condition.
\end{proof}

\begin{lemma}\label{lem:phasecolor}
The algorithm of \cite{hknt_local_d1lc} for \DILC for nodes of degree at least $\log^7 n$, running on a graph $G$, of maximum degree \emph{at most} $n^{7\delta}$, can be derandomized in $O(\log^* n)$ rounds. The process uses $O(n^{7\delta cC})$ space per machine and $O(n_G \cdot n^{7\delta cC})$ global space, where $C$ is as in \Cref{lem:phasederand}.
\end{lemma}

\begin{proof}
We use $\Delta_G = n^{7\delta}$ as an upper bound on the maximum degree $G$, and first compute the $O(\Delta_G^{8c})$-coloring of $G^{4c}$ required for \Cref{lem:fullderand}. This can be done in $O(\log^* n)$ rounds by simulating Linial's \cite{Linial92} deterministic \LOCAL algorithm round-by-round. Then, since we showed in \Cref{lem:derandomizable-subroutines} that the algorithm of \cite{hknt_local_d1lc} can be expressed as a sequence of $O(\log^* n)$ \emph{phases}, each of which are normal $(c, \Delta_G )$-round distributed procedures for some constant $c$, we can apply \Cref{lem:fullderand} to derandomize each phase in turn, resulting in a deterministic coloring of all nodes.
\end{proof}

Since the algorithm of \cite{hknt_local_d1lc} is only for nodes of degree at least $\log^7 n$, note that our repeated derandomization steps can leave a set $D$ of remaining uncolored nodes with degrees of at most $\log^7 n$.

\subsection{\DILC when the maximum degree is $n^{7\delta}$}

The remaining algorithm is simple: we apply \Cref{lem:phasecolor} to deterministically color all nodes of degree at least $\log^7 n$ (with some nodes potentially remaining uncolored once their uncolored degree drops below $\log^7 n$, and then apply the following lemma to color the remaining low-degree nodes:
\begin{lemma}[Lemma 14 of \cite{CDP21}]\label{lem:lowdeg}
For any $n$-node graph $G$ with maximum degree $\Delta = \log^{O(1)} n$, there exists an $O(\log \log \log n)$-round deterministic algorithm for
computing \DILC, using $O(n^\phi)$ space per machine and $O(n^{1+\phi})$ global space, for any positive constant~$\phi \in (0,1)$.
\end{lemma}

The algorithm for \DILC when the degree is $O(n^{7\delta})$ is described in \Cref{alg:DLDC} and its correctness is proved in \Cref{thm:midcolor}.

\begin{algorithm}[H]
	\caption{\textsc{DerandomizedMidDegreeColor}$(G)$}
	\label{alg:DLDC}
	
		    Let $G_{\text{low}}$ consist of all nodes of $G$ with palette size at most $\log^7 n$.
		
		    Derandomize coloring of $G\setminus G_{\text{low}}$ as in \Cref{lem:phasecolor}, leaving a set $D$ of uncolored nodes with low degree.
		
		    
		
		    $G_{\text{low}}\gets G_{\text{low}} \cup D$.
	Update palettes of $G_{\text{low}}$, then color using \Cref{lem:lowdeg}.

\end{algorithm}

\begin{theorem}\label{thm:midcolor}
\textsc{DerandomizedMidDegreeColor}, performed on a DL1C instance $G$ of degree at most $n^{7\delta}$, properly colors all nodes in $O(\log \log\log n)$ rounds of \MPC, using $O(n^{7\delta cC})$ space per machine and $O(n_{G} \cdot n^{7\delta cC})$ global space, where $C$ is as in \Cref{lem:phasederand}.
\end{theorem}

\begin{proof}
After applying \Cref{lem:phasecolor} the degree of all uncolored nodes in $G$ must also be at most $\log^7 n$, so all remaining nodes are colored by \Cref{lem:lowdeg}.

The space usage is dominated by that of \Cref{lem:phasecolor}, and the number of rounds required is $O(\log\log\log n)$ since it is dominated by the $O(\log\log\log n)$ rounds for \Cref{lem:lowdeg}.
\end{proof}

%\section{Overall Deterministic D1LC Algorithm for Sublinear-Space \MPC}
\section{Deterministic D1LC Algorithm}

To reduce our \DILC instances to a collection of instances with lower degree, in order to fit constant-radius balls onto machines, we employ a recursive structure \textsc{LowSpaceColorReduce} (\Cref{alg:LSColorReduce}) similar to \cite{CDP20,CDP21}.

\begin{algorithm}[H]
	\caption{\textsc{LowSpaceColorReduce}$(G)$}
	\label{alg:LSColorReduce}
		$G_{\text{mid}},G_1 \dots, G_{n^{\delta}} \gets \textsc{LowSpacePartition}(G)$.
		
	    For each $i = 1, \dots,n^{\delta}-1$ in parallel: call \textsc{LowSpaceColorReduce}$(G_i)$.
	
		Update color palettes of $G_{n^{\delta}}$, call \textsc{LowSpaceColorReduce}$(G_{n^{\delta}})$.
		
		Update color palettes of $G_{\text{mid}}$.
		
		Color $G_{\text{mid}}$ using \textsc{DerandomizedMidDegreeColor}$(G_{\text{mid}})$.
\end{algorithm}

The recursive structure in the above algorithm relies on a partitioning procedure to divide the nodes and colors in the input instance into \emph{bins}:

\begin{algorithm}[H]
	\caption{\textsc{LowSpacePartition}$(G)$}
	\label{alg:LSPartition}
		Let $G_{\text{mid}}$ be the graph induced by the set of nodes $v$ with $d(v)\le n^{7\delta}$.
		
		Let hash function $h_1:[n]\rightarrow [n^{\delta}]$ map each node $v$ to a bin $h_1(v) \in [n^{\delta}]$.
		
		Let hash function $h_2:[n^2]\rightarrow [n^{\delta}-1]$ map colors $\gamma$ to a bin $h_2(\gamma) \in [n^{\delta}-1]$.
		
		Let $G_1,\dots,G_{n^{\delta}}$ be the graphs induced by bins $1,\dots,n^{\delta}$ respectively, minus the nodes in $G_{\text{mid}}$.
		
		Restrict palettes of nodes in $G_1,\dots,G_{n^{\delta}-1}$ to colors assigned by $h_2$ to corresponding bins.
    	
    	Return $G_{\text{mid}},G_1,\dots,G_{n^{\delta}}$.
\end{algorithm}


% The idea is that, so long as node degrees are at least $n^{7\delta}$,  randomly assigning them to bins is sufficient to ensure that the number of their neighbors mapped to the same bin will concentrate around the expectation, even if the choices are only $O(1)$-wise independent. Then, hash functions that guarantee such a property can be chosen from $O(1)$-wise independent families using the method of conditional expectations as in \cite{CDP20}. Of course, there will still be some error, so if we randomly partition the available colors among the bins in the same way, then palette size will no longer necessarily be larger than degrees. However, as used in \cite{CFGUZ19,CDP20,CDP21}, it transpires that leaving a single bin without colors, and partitioning the colors among the other bins, is enough to outweigh this error and provide a sufficiently large palette to each node with high probability. The induced graphs of the bins with colors can then be recursively colored in parallel (since they use disjoint palettes), and the remaining bin can be colored afterwards (with nodes using their original palettes minus the colors that have been used already by their neighbors in other bins). This remaining bin can always be colored, since a valid partial coloring of a D1LC instance leaves the rest of the graph alsa $(\deg + 1)$-list colorable.
% \sams{might be worth clarifying that this is still a D1LC instance}.



We can follow the analysis of \cite{CDP20} to analyze the partitioning process, since it is only the base cases that have changed. The following lemma provides the important properties of the partitioning:

\begin{lemma}[Lemma 4.6 of \cite{CDP20}]\label{lem:LSdeterministic-hashing}
Assume that, at the beginning of a call to \textsc{LowSpacePartition}, we have $d(v)<p(v)$ for all nodes $v$. Then, in $O(1)$ \MPC rounds with $O(n^{7\delta})$ local space per machine and $O(n+m)$ global space (over all parallel instances), one can deterministically select hash functions $h_1$, $h_2$ such that after the call,
	%
	\begin{itemize}
		\item for any node $v\notin G_{\text{mid}}$, $d'(v) < 2d(v)n^{-\delta}$, and
		\item for any node $v$, $d'(v)<p'(v)$.
	\end{itemize}
 Here $d'(v)$ denotes the degree of $v$ in the subgraph induced by the nodes present in the same bucket as $v$ and $p'(v)$ denotes the number of $v$'s palette colors that are in the same bucket as $v$.
\end{lemma}

Now we are ready to prove our main result that $(\deg+1)$-list coloring can be performed deterministically in $O(\log \log\log n)$ rounds of \MPC, with $O(n^\spacexp)$ local space and $O(m+n^{1+\spacexp})$ global space.

\begin{proof}[Proof of \Cref{thm:main:deter}]
%
As in \cite{CDP21}, calling \textsc{LowSpaceColorReduce} on our input graph creates a recursion tree of $O(1)$ depth (since each recursive call reduces the maximum degree by a $n^{-\delta}$ factor). It therefore creates $O(1)$ sequential sets of base-case instances to solve concurrently, which in \Cref{alg:LSColorReduce} are solved by \textsc{DerandomizedMidDegreeColor}. Furthermore, each set of concurrent instances has at most $n$ nodes in total, since all nodes are only partitioned into one instance, and each instance has maximum degree $n^{7\delta}$.

By \Cref{thm:midcolor}, each such instance $G$ is colored in $O(\log\log\log n)$ rounds using $O(n^{7\delta cC})$ space per machine and $O(n \cdot n^{7\delta cC})$ global space. The global space used by all concurrent instances is therefore $O(n \cdot n^{7\delta cC})$. Setting $\delta$ sufficiently smaller than the space parameter \spacexp, this is $O(n^\spacexp)$ space per machine and $O(n^{1+\spacexp})$ global space. Since receiving the input and the first call to \textsc{LowSpacePartition} also requires $O(m)$ global space, the overall space bound is $O(m+n^{1+\spacexp})$.
\end{proof}


%Now, we discuss about a randomized faster algorithm when the minimum degree of the graph is at least $\log ^7 n$. Note that, in this case, the algorithm of \cite{hknt_local_d1lc} takes $O(\log^* n)$ rounds in \textsc{Local}. So, if we are happy with randomized algorithm, we can first design one  similar to \textsc{DerandomizedMidDegreeColor} when the degree lies in $[\log^7 n, n^{7\delta}]$ such that $G_{\text{low}}$ is empty and there is no deferred node in the first iteration. Note that this algorithm will require $O(\log ^*n n)$ rounds. Then due to 
%\input{delta.tex}
%\input{Coloring-delta.tex} 

==> parts/d1lc_linear_space.tex <==
\section{D1LC in Sublinear \MPC with Linear Global Space}
